Continuous Control with Contexts, Provably

A fundamental challenge in artificial intelligence is to build an agent that generalizes and adapts to unseen environments. A common strategy is to build a decoder that takes the context of the unseen new environment as input and generates a policy accordingly. The current paper studies how to build a decoder for the fundamental continuous control task, linear quadratic regulator (LQR), which can model a wide range of real-world physical environments. We present a simple algorithm for this problem, which uses upper confidence bound (UCB) to refine the estimate of the decoder and balance the exploration-exploitation trade-off. Theoretically, our algorithm enjoys a $\widetilde{O}\left(\sqrt{T}\right)$ regret bound in the online setting where $T$ is the number of environments the agent played. This also implies after playing $\widetilde{O}\left(1/\epsilon^2\right)$ environments, the agent is able to transfer the learned knowledge to obtain an $\epsilon$-suboptimal policy for an unseen environment. To our knowledge, this is first provably efficient algorithm to build a decoder in the continuous control setting. While our main focus is theoretical, we also present experiments that demonstrate the effectiveness of our algorithm.

==> meta_algo.tex <==
\paragraph{New algorithm}
We summarize our meta-RL framework.
\begin{enumerate}
\item Observe a context.
\item Play an episode. Record the experience and transfer the experiences using the context.
\item Learn the meta parameters based on the transfered parameters.
\end{enumerate}

\paragraph{Old algorithm}
In this section we describe our general framework.
At high level, the algorithm is very simple.
Suppose we observe $N$ $\mdp$s and each MDP we collect $n$ trajectories.
We estimate linear mapping using the following straightforward procedure.
\begin{itemize}
\item For each $\mdp_k$, we use a solver~\cite{yang2019reinforcement} to obtain an estimate of the transition core $\widehat{\mat{M}}_k$.
\lin{Need some additional assumption to guarantee the performance of $\widehat{\mat{M}}$}
\item Solve the following regression problems, \begin{align}
	\widehat{T} = \argmin_{\linopt: \mathbb{R}^{\dmdp} \rightarrow \mathbb{R}^{d\times d'}} \frac{1}{2N}\norm{\linopt(\vect{x}_k)-\widehat{\mat{M}}_k}_F^2
\end{align}
\simon{Is Frobenius norm the right way?}
\end{itemize}
\simon{This algorithm is a parallel version. In the sequential version, is it possible to reduce the sample complexity?}

Our main result is the following theorem which shows our prediction on the transition core is accurate.
\begin{thm}[Main Theorem]
	\label{thm:main}
If $N = \Omega\left(blah\right)$ and $n = \Omega\left(blah\right)$, then with probability at least $1-\delta$ over training data we have \begin{align}
\expect_{\mdp \sim \distmdp} \norm{\widehat{\linopt}\left(x\right) - M}_F^2 \le \epsilon.
\end{align}
where $M$ is the transition core of $\mdp$.
\end{thm}

If we also do reward transfer, we can obtain the following guarantee on the zero shot reinforcement learning.
$V^{\pi}$ is the induced policy by $\widehat{\linopt}$ and some reward transfer and $s_1$ is a fixed starting state.
\begin{cor}
If $N = \Omega\left(blah\right)$ and $n = \Omega\left(blah\right)$, then with probability at least $1-\delta$ over training data we have \begin{align}
\expect_{\mdp \sim \distmdp} \left[V^{\pi}(s_1)-V^*(s_1)\right] \le \epsilon.
\end{align}
\end{cor}




